Optimization Algorithms for Improving the Performance of Permutation Trellis Codes

In this paper, soft-decision (SD) decoders of permutation trellis code (PTC) with $M$-ary frequency shift keying are designed using three optimization algorithms and presented in four decoding schemes. In a concatenated code such as PTC, the Viterbi decoder for the outer convolutional code provides maximum likelihood decoding. Hence, the error correction performance is dependent on the decoding scheme used for the inner code. Due to the structure of the encoder with the modulation scheme, the channel output can be interpreted as an assignment problem. SD decoding can then be designed accordingly, using the presented, low-complexity optimization-based schemes. The bit error rate (BER) performance of the schemes are simulated in an additive white Gaussian noise (AWGN) and powerline communication (PLC) channel. The complexities of the schemes are also presented. The performance of the SD schemes are compared with the existing SD threshold detector, with BER results showing significant coding gain for certain codebooks. From the results, a reasonable trade-off between the complexity and coding gain is observed for a noisy channel such as the PLC channel.

==> content.tex <==
% IEEEtran.cls defaults to using nonbold math in the Abstract.
% This preserves the distinction between vectors and scalars. However,
% if the journal you are submitting to favors bold math in the abstract,
% then you can use LaTeX's standard command \boldmath at the very start
% of the abstract to achieve this. Many IEEE journals frown on math
% in the abstract anyway.

% Note that keywords are not normally used for peerreview papers.
%\begin{IEEEkeywords}
%$M$-FSK, Permutation codes, Permutation trellis, Soft-decision decoding, Viterbi decoding algorithm.
%\end{IEEEkeywords}


\maketitle

\section{Introduction}

%Several methods regarding the construction of permutation trellis codes have been studied and reported in \cite{ferreira-wright-nel, chang-chen-klove-tsai, ferreira-vinck-swart-beer}. 
Permutation Trellis codes (PTC) reported in \cite{ferreira-vinck, ferreira-vinck-swart-beer} illustrate the combination of permutation codes with convolutional codes of different code rates, constraint lengths and minimum free distance. The PTC are obtained by using different one-to-one mappings such that the Hamming distance between any two binary sequences and their corresponding permutation sequences are preserved, increased or decreased \cite{ferreira-vinck, chang-chen-klove-tsai, ferreira-vinck-swart-beer}. PTC can be decoded using hard-decision or soft-decision \cite{proakis} using the Viterbi algorithm \cite{viterbi}. %in general achieves maximum likelihood (ML) decoding performance for convolutionally encoded sequences. %In PTC, the convolutionally encoded binary sequences are mapped onto a permutation of non-binary integers. 
The decoder proposed in \cite{ferreira-vinck-swart-beer} reduces the decoding complexity for a power line communication (PLC) channel by modifying the branch metric of the Viterbi decoder.

%Asides the combination of permutation codes 
%Error performance is one of the major characteristic that defines the effectiveness of permutation codes and contribute to the overall system performance. Therefore, extensive evaluation of these codes is very important and different results have been reported by researchers. 
Error performance evaluation of permutation codes has been conducted in conjunction with some modulation schemes in a bid to achieve overall excellent system performance. For example, to combat narrow-band interference (NBI) and impulse noise (IN) in a PLC channel, $M$-ary Frequency Shift Keying ($M$-FSK) along with permutation codes was recommended in \cite{ferreira-vinck, ferreira-vinck-swart-beer} and \cite{vinck}. In cognitive radio networks, PTC with $M$-FSK in \cite{bardan-masazade-ozdemir-han-varshney}, finds an appropriate mapping in order to increase the data rate of secondary users at low power in the presence of narrow-band interference by primary users. In another study, the use of PTC in conjunction with quadrature amplitude modulation (QAM) and quadrature phase shift-keying (QPSK) was reported \cite{gagnon-haccoun}. In these schemes, an appropriate mapping of the binary output of the convolutional encoder to a suitable permutation code book increases the distance between the constellation points. 
$M$-FSK allows non-coherent detection, using the square law or envelope detection (ED) to select the signal with the highest energy from a pair of $M$ quadrature correlators at each sampling period \cite{proakis}. However, the resulting non-binary sequence is not always a permutation of all the integers of a codeword in the case of a permutation-coded $M$-FSK. As a result, the demodulated non-binary sequence forwarded to the non-binary Viterbi decoder may have the same Hamming distance with multiple branches at each stage in the trellis, hence leading to a decoding error. Also, decoding the non-binary sequence with hard-decision requires a look-up table in order to find a permutation sequence with the least Hamming distance with the demodulated sequence. In such case, the received sequence may have the same Hamming distance with more than one codeword and when the size of the code book is large, the hard-decision operation becomes too complex. The permutation soft-decision decoder (PSDD) in \cite{kolade-versfeld-van-wyk} decodes permutation block codes with $M$-FSK at reduced complexity using two optimization algorithms. The algorithms are combined to present an iterative decoder which improves BER performance when compared with the hard-decision decoder.

\begin{figure}
\centering\includegraphics[width=20pc]{diagrams/system_model_encoder.eps}
\caption{System model for permutation trellis encoder.}
\label{fig:permutation-trellis-system-model}
\end{figure}

In this paper, optimization algorithms are presented as soft-decision decoders PTC with $M$-FSK. 
First, the branch-and-bound (BB) algorithm is introduced as a novel SD decoder. In addition, the iterative PSDD in \cite{kolade-versfeld-van-wyk} is implemented as a PTC decoder. Results show that the additional step of converting the SD output to its binary equivalent before decoding with the Viterbi algorithm produces better BER performance for both decoders. The complexity of the decoders are also presented and in some cases, the SD decoder reduces the decoding complexity for large codebooks while simultaneously improving the BER performance.
%While the iterative PSDD in \cite{kolade-versfeld-van-wyk} is implemented in PTC and presented in two schemes, branch-and-bound (BB) is further introduced as a novel SD decoder and also presented in two schemes. Results show that the scheme which uses a non-binary to binary demapper step in the decoder improves the BER performance, although at additional complexity. However, in cases where a threshold detector is used, the complexity of the decoder is reduced in comparison with the existing decoder in \cite{ferreira-vinck-swart-beer}.

%In this paper, we report an improvement in the BER coding gain performance of PTC modulated with $M$-FSK by using optimization algorithms to decode the soft output of the channel. Branch and bound (BB) and the iterative soft-decision (SD) decoder in \cite{kolade-versfeld-van-wyk} are presented in two schemes each. While both SD decoders produce a permutation non-binary sequence, the first scheme forwards the permutation sequence to a non-binary Viterbi decoder. The second scheme converts the permutation sequence to its binary equivalent before forwarding to the binary Viterbi decoder. The BER improvement of the schemes is however at the expense of complexity for small-sized code books. However, the schemes can provide an attractive trade-off between complexity and the BER coding gain when decoding large-sized code books.

%Also, the correlators required for demodulating $M$-FSK are eliminated, thereby reducing circuitry complexity. % When combined with PTC, it further reduces the decoding complexity while improving the coding gain.
%In this paper, we report an improvement in the coding gain performance of PTC modulated with $M$-FSK by using optimization algorithms to iteratively decode the soft output of the channel. To begin with, we apply the branch-and-bound optimization algorithm as a new soft-decision decoder using two schemes. In the first scheme, the permutation sequence produced by the soft-decision decoder is forwarded to the Viterbi decoder which is modified to decode non-binary sequences. The second scheme converts the permutation sequence to its binary equivalent or "demapping" and forwards the binary sequence to the Viterbi decoder. In addition, we extend the soft-decision decoder presented in \cite{kolade-versfeld-van-wyk} to PTC in two new but similar schemes as applied to the branch-and-bound schemes. The optimization algorithms presented always output a permutation sequence and more iterations increase the probability of producing a codeword in the encoder's code book. As a result, the permutation sequence forwarded to the Viterbi decoder has a zero Hamming distance with only one of the branches at each stage in the trellis. If the permutation sequence is demapped before forwarding to the Viterbi decoder, then the equivalent binary sequence follows a path in the trellis with zero Hamming distance. In these schemes, the more the iterations in the PSDD, the higher the probability of producing a sequence in the code book hence improving the coding gain performance. Furthermore, the soft-decision decoders' coding gain performance approaches ML performance as the code book size increases with respect to the size of all possible codewords for the selected code book. The coding gain improvement of the schemes is however at the expense of complexity for small size code books but can provide an attractive trade-off between complexity and coding gain when decoding large-sized code books. %Also, the correlators required for demodulating $M$-FSK are eliminated, thereby reducing circuitry complexity. % When combined with PTC, it further reduces the decoding complexity while improving the coding gain.

%The rest of the paper is organized as follows: In Section II, the system model is presented. In Section III, the three optimization algorithms are discussed, in relation to the four proposed schemes and the results are presented in Section IV. Finally conclusions are given in Section V.

\section{System Model}
\subsection{Permutation Trellis Codes}
Permutation trellis codes combine convolutional codes and permutation codes at the encoder and uses a modified Viterbi decoder to decode the demodulated signal. The convolutional encoder with constraint length $K$ first encodes the incoming message in Fig. \ref{fig:permutation-trellis-system-model} by shifting $k$ binary bits of information via a linear shift register consisting of $K$ stages. The output is a corresponding $n$ bit binary sequence, hence a code rate of $R_{\text{C}} = k/n$. Each $n$-tuple from the convolutional encoder is then mapped onto a permutation codeword $\boldsymbol{c} = c_1 c_2 \dots c_M$ of length $M$ such that $n \leq M$. Each codeword belongs to a code book $C$ which consists of $2^n$ unique codewords and $C$ is a subset of the set of all possible permutations consisting of $M!$ codewords. Therefore, the combined code rate is $R_{\text{P}} = k/M$.
%Permutation trellis \cite{ferreira-vinck-swart-beer} are constructed by combining convolutional codes with permutation codes. As shown in fig. \ref{fig:permutation-trellis-system-model}, convolutional codes are used as the outer code for permutation codes such that an $n-$tuple binary output of the convolutional encoder is mapped onto the permutation codeword of length $L$. 
The mapping is done such that the Hamming distance between each binary sequence and its respective permutation sequence is preserved, reduced or increased. An example of a distance increasing mapping (DIM) is $\{00 \mapsto 231, 01 \mapsto 213, 10 \mapsto 132, 11 \mapsto 123\}$ where $n = 2, M=3$ and $\{000 \mapsto 1234, 001 \mapsto 1342, 010 \mapsto 1423, 011 \mapsto 3241, 100 \mapsto 4132, 101 \mapsto 2314, 110 \mapsto 2431, 111 \mapsto 2143\}$ where $n = 3, M=4$. We refer the reader to other examples of DIMs, distance reducing mappings and distance preserving mappings in \cite{ferreira-vinck, ferreira-vinck-swart-beer, chang-chen-klove-tsai}.

%The maximum likelihood decoding of a  convolutional code uses a Viterbi decoder and the upper bound of the bit error probability is defined as \cite{proakis}

%\begin{equation}
%  \label{eq:pe-convolutional-code}
%    P_e \leq \sum_{d=d_{\text{free}}}^{\infty} a_dP_2(d),
%\end{equation}
%where \begin{equation} 
%	\label{eq:probability-of-error-convolutional-code}
%	P(d) = \frac{1}{2} {d \choose \frac{d}{2}} p^{d/2}(1 - p)^{d/2} + \sum_{k = d/2+1}^{d} {d \choose k} p^k (1 - p)^{n - k}  
%end{equation}
%when $d$ is even and $p = \frac{1}{2} \text{exp} (-\frac{1}{2} R_{\text{C}} \text{SNR} )$ which represents the probability of error when the bits in each codeword are transmitted using FSK and noncoherently detected. If $d$ is odd, the second term in (\ref{eq:probability-of-error-convolutional-code}) is ignored. $a_d$ describes the paths with Hamming distance $d$ bits when compared with the transmitted codeword, $P_2(d)$ describes the probability of the decoded path having Hamming distance of $d$ bits with the transmitted codeword. The code's free distance $d_{\text{free}}$ describes the Hamming distance between the all-zero path in the trellis and a trellis path which departs the all-zero path and returns to the all zero path.

%\begin{equation}
%  \label{eq:pe-ptc}
%    P_e(\boldsymbol{c}) \leq \sum_{d=d_{\text{free}}^{'}}^{d_{\text{free}}^{'}+z} a_{d}^{\boldsymbol{c}}P_{2}^{\boldsymbol{c}}(d),
%\end{equation}
%where $a_{d}^{\boldsymbol{c}}$ and $P_{2}^{\boldsymbol{c}}(d)$ are similar to $a_d$ and $P_2(d)$ in (\ref{eq:pe-convolutional-code}) but correspond to the permutation codeword $\boldsymbol{c}$ mapped to a convolutional codeword, $d_{\text{free}}^{'}$ is the free distance of the combined code and $z \in \mathbb{N}$ describes the $z+1$ paths.
%where $a_{d}^{\boldsymbol{c}}$ describes the paths with hamming distance $d$ bits when compared with the transmitted permutation codeword $\boldsymbol{c}$ and $P_{2}^{\boldsymbol{c}}(d)$ describes the probability of the decoded path having hamming distance of $d$ bits with the transmitted permutation codeword.
%\begin{equation}
%    P_{2}^{\boldsymbol{c}}(d) = 
%    \begin{dcases}
%        \sum_{d={\frac{d}{2} + 1}}^{d} \prod_{v=1}^{V} P(\boldsymbol{R} | \boldsymbol{T}), \:\:\:\:\:\:\:\:\:\:\:\: \text{ odd } d,\\
%        \frac{1}{2} \prod_{v=1}^{V} P(\boldsymbol{R} | \boldsymbol{T}) \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{even } d \\ + \sum_{d={\frac{d}{2} + 1}}^{d} \prod_{v=1}^{V} P(\boldsymbol{R} | \boldsymbol{T}),
    %\end{dcases}
%\label{eq:definition-of-P2d}
%\end{equation}

\subsection{$M$-ary Frequency Shift Keying with PTC}

Consider a set of $M$ orthogonal signals $\boldsymbol{s}_{1}, \boldsymbol{s}_{2}, \dots, \boldsymbol{s}_{M}$, %each of length $M$ 
each having one of the $M$ different frequency components and a low pass vector representation \cite{proakis} 
\begin{align*}
    \boldsymbol{s}_{m} &= (\underbrace{0,\dots,0}_{m-1},\sqrt{2E_s}, \underbrace{0, \dots, 0}_{M-m})^T.
\end{align*}
The notation $(\cdot)^T$ denotes the transpose operation and the symbol energy $E_s$ is in the $m$-th ($m = 1, 2, \dots, M$) element denoting the $m$-th frequency. The permutation sequence in Fig. \ref{fig:permutation-trellis-system-model} is modulated using the $M$ orthogonal vectors such that each symbol in the sequence has a one-to-one mapping with an $M$-FSK vector $\boldsymbol{s}_{m}$. Therefore, the $M$-FSK-modulated permutation sequence in Fig. \ref{fig:permutation-trellis-system-model} produces $\boldsymbol{S} = [s_{ij}] \in \{0, 1\}^{M \times M}$, which consists of a permutation of all vectors $\boldsymbol{s}_{1}, \boldsymbol{s}_{2}, \dots, \boldsymbol{s}_{M}$. Each vector $\boldsymbol{s}_{m}$ represents a column in $\boldsymbol{S}$ and appears once in every $M$ block. Therefore, it is obvious the modulated permutation sequence utilizes all $M$ available frequencies. %Note that each 

Assuming an additive white Gaussian noise (AWGN) channel and that the phase $\phi$ is unknown at the receiver, each vector is non-coherently received at each time slot as
\begin{equation}
  \label{eq:awgn-equation}
  \begin{aligned} 
    \boldsymbol{y} &= e^{j\phi} \boldsymbol{s}_{m} + \boldsymbol{v}_{\text{G}},
  \end{aligned}
\end{equation}
where $\phi$ is a random variable and is distributed uniformly between 0 and $2\pi$ while $\boldsymbol{v}_{\text{G}}$ is a complex-valued Gaussian distribution $\mathcal{C}\mathcal{N} (0,2N_0)$. In the presence of IN such as in a PLC channel, each transmitted vector is received as
\begin{equation}
  \label{eq:awgn-equation}
  \begin{aligned} 
    \boldsymbol{y} &= e^{j\phi} \boldsymbol{s}_{m} + \boldsymbol{v}_{\text{G}} + \boldsymbol{v}_{\text{I}} \sqrt{\boldsymbol{p}}.
  \end{aligned}
\end{equation}
The noise vector $\boldsymbol{v}_{\text{I}}$ models the IN as complex variables with Gaussian distribution $\mathcal{C}\mathcal{N} (0,\frac{2N_0}{A})$ and $\boldsymbol{p}$ is a Poisson-distributed random sequence whose values are determined by the impulsive index $A$. NBI is also a common noise source in PLC. While IN may affect some or all frequencies in a time slot, NBI may affect one of the $M$ frequencies over a period of time as illustrated in \cite{ferreira-vinck-swart-beer}.
Each received $M$-FSK vector $\boldsymbol{y}$ at each time slot is demodulated by choosing the $\boldsymbol{s}_{m}$ with the highest envelope
\begin{equation} 
  \begin{aligned}
    \label{eq:mfsk-envelope-detector}
%    \[\hat{s} = \argmax_{x \in \mathcal{X}} |r^H f_i|^2\]
    \hat{r} = \displaystyle\arg \max_{m \in M}} |\boldsymbol{y}^H \cdot \boldsymbol{s}_{m}|.
  \end{aligned}
\end{equation}
This produces an integer $\hat{r}$ which is equivalent to the likely transmitted $m$-th frequency.

\subsection{Hard-Decision Decoder}
The received $M$-FSK modulated permutation sequence $\boldsymbol{Y} = [y_{ij}] \in \mathcal{C}^{M \times M}$ is equivalent to the transmitted $\boldsymbol{S}$ and consists of a permutation of column vectors $\boldsymbol{y}_1, \boldsymbol{y}_2, \dots, \boldsymbol{y}_M$. Demodulating each column in $\boldsymbol{Y}$ using (\ref{eq:mfsk-envelope-detector}) produces a permutation of integers $\hat{\boldsymbol{r}} = \hat{r}}_1 \hat{r}}_{2} \dots, \hat{r}}_{M}$. The branch metric in the Viterbi decoder is then modified by comparing and choosing the minimum Hamming distance $\displaystyle \min_{\boldsymbol{c}_q \in C}} d (\boldsymbol{\hat{r}}, \boldsymbol{c}_q)$ between $\hat{\boldsymbol{r}}$ and $\boldsymbol{c}_q$ for $1 \leq q \leq 2^n$ on each transition path of the trellis. We hence refer to this decoder as the PTC decoder.

The envelope detector in (\ref{eq:mfsk-envelope-detector}) is not optimal in scenarios such as in the PLC channel where large envelopes are detected at the demodulator as a result of IN and NBI \cite{schaub}. A more adequate threshold detector proposed in \cite{ferreira-vinck-swart-beer} sets a threshold of $0.6\sqrt{E_m}$ on the symbol energy $E_m$ of each received sample, such that samples above the threshold are demodulated as one while values below the threshold are demodulated to zero. This results in an $M \times M$ matrix which is then compared with all possible transmitted codeword matrices and the branch metric is computed as 
%The hard-decision decoder hence finds the codeword $\boldsymbol{c}$ with the minimum Hamming distance $d_{\text{m}} = \displaystyle \min_{\boldsymbol{c}_i \in C}} d (\boldsymbol{\hat{y}}, \boldsymbol{c}_i)$ with $\hat{\boldsymbol{y}}$.
%The PTC decoder performs a hard-decision and is valid for different $n$ to $M$ mappings. 
\begin{equation} 
  \begin{aligned}
    \label{eq:ptc-decoder-branch-metric}
    M - [\sum_{1 \leq i, j\leq M} (s_{ij} \land y_{ij})],
  \end{aligned}
\end{equation}
for each branch where the notation $\land$ is the binary AND operation. Then, the branch with the minimum metric value is chosen. We hence refer to this decoder as the PTC threshold decoder.

\subsection{The Permutation Soft-Decision Decoder}
Each codeword $\boldsymbol{c}_q$ produces a matrix $\boldsymbol{S}$ %, x_{it} \ge 0$ 
such that
\begin{equation} 
    \label{eq:assignment-problem-explained}
    \begin{aligned} 
      \sum_{i=1}^{M} s_{ij} = \sum_{j=1}^{M} s_{ij} = 1, 
      %(i = 1, \dots, M), \\
      %\sum_{i=1}^{M} s_{it} = 1, (t = 1, \dots, M),
    \end{aligned}
\end{equation}
%\begin{equation} 
%    \label{eq:assignment-problem-explained}
%    \begin{aligned} 
%      \sum_{i=1}^{M} s_{it} = 1, \:\:\: \:\:\:
%      \sum_{t=1}^{M} s_{it} = 1, 
%    \end{aligned}
%\end{equation} %for $x_{it} \ge 0$ 
for $i = 1,2, \dots, M$, $j = 1,2, \dots, M$. % and is a solution to an assignment problem.
If $\boldsymbol{Y}$ is considered as a soft input to the PSDD \cite{kolade-versfeld-van-wyk}, then the PSDD decodes $\hat{\boldsymbol{Y}} = [\hat{y}_{ij}] \in \mathcal{C}^{M \times M}$ at the first iteration $g = 1$ by finding the cost $Z_1$ that minimizes

\begin{equation} 
    %Z_1 = \sum _{i=1}^{M} \sum _{t=1}^{M} y_{it} x_{it}, \\ 
    Z_1 = \sum_{i=1}^{M}\sum_{j=1}^{M} \hat{y}_{ij} s_{ij},%, \quad \mbox{for} \ Z_1 \leq Z_g \leq Z_{2^n}.
\end{equation}
subject to (\ref{eq:assignment-problem-explained}) and $\hat{y}_{ij} = -|y_{ij}|$.
The Hungarian Algorithm (HA) \cite{kuhn} can find the matrix $\boldsymbol{S} = [s_{ij}]$ that produces the minimum cost $Z_1$ with a corresponding permutation sequence 
\begin{equation} a_1 = {\{(1, j_1), (2, j_2), \dots, (M, j_{M})}\}, \end{equation}
where $j_1, j_2, \dots, j_M$ is a permutation of symbols $1, 2, \dots, M$. If $a_1$ produces a codeword $\boldsymbol{c} \notin C$, the Murty's algorithm \cite{murty} ranks $Z_2, Z_3, \dots, Z_{2^n}$ to find a codeword $\boldsymbol{c} \in C$. Using the solution matrix from $Z_1$, $n-1$ non-empty subsets of $\boldsymbol{Y}$ form nodes $N_1, N_2, \dots, N_{n-1}$, by partitioning $a_1$. Nodes in this case are defined as $N_1 = {\{\overline{(1, j_1)}}\},N_2 = {\{(1, j_1), (\overline{2,j_2)}}\},\dots, N_{n-1} = {\{(1, j_1), \dots, \overline{(n-1, j_{n-1})}}\}$. Row-column pairs with the bar ($\overline{\cdot,\cdot}$) indicate row-column elements to be replaced with $\infty$ while row-column elements without the bar are removed from $\boldsymbol{Y}$. The minimum cost is then solved for each node and the node with the least cost forms the next assignment $a_2$.
 %As will be explained in the following sections, the permutation sequence produced by the PSDD can either be decoded directly by the modified Viterbi decoder or demapped to binary using the mapping table before decoding with the Viterbi decoder.  %Depending on the number of iterations, it is possible to produce a non-binary sequence with zero Hamming distance with at least one transition path in the trellis. 
%In the next section, we describe in detail operations of the soft-decision decoder and two methods of combining the soft-decision decoder with the trellis decoder.
%\subsection{The Permutation Soft-decision Decoder}
%As mentioned earlier, a permutation codeword utilizes all $M$ possible frequencies when modulated with $M$-FSK. 
%Therefore, if signals $\boldsymbol{s}_{1}, \boldsymbol{s}_{2}, \dots \boldsymbol{s}_{M}$ are arranged as column vectors, modulating a codeword with $M$-FSK produces a matrix $\boldsymbol{S} = [s_{it}] \in \{0, 1\}$ that is a permutation of all the signals and
%\begin{equation} 
%    \label{eq:assignment-problem-explained}
%    \begin{aligned} 
%      \sum_{i=1}^{M} s_{it} = 1, (i = 1, \dots, M), \\
%      \sum_{i=1}^{M} s_{it} = 1, (t = 1, \dots, M).
%    \end{aligned}
%\end{equation}
%Each column represents the signal transmitted at each signalling time $t$.
 %Each column in $S$ represents the vector $\boldsymbol{s}_m$ which is transmitted at each time instant $t$. However, at the output of the channel, the corrupted sequence must be rearranged into an $M \times M$ matrix and each column represents the corrupted $M$-FSK vector at $t$. %As an example, each symbol in a permutation codeword (4123) is mapped onto a unique $M$-FSK vector using a modified modulator which outputs a matrix
%\[S = \left[ \begin{array}{cccc}
%0 & 1 & 0 & 0 \\
%0 & 0 & 1 & 0 \\
%0 & 0 & 0 & 1 \\
%1 & 0 & 0 & 0 \end{array} \right].\] 
%At the output of the AWGN channel, the received modulated permutation sequence is an $M \times M$ matrix $\boldsymbol{Y} = [y_{it}] \in \mathbb{R}^{+}$. %which corresponds to an $M$-FSK vector 
%and each component $y_{it}$ is defined as
%and $v$ is a random complex-valued Gaussian sample from (\ref{eq:awgn-equation}). 

The PSDD makes an optimal decision (OD) by using a brute force to find the codeword $\boldsymbol{c}$ from all possible permutations with the highest cost
\begin{equation} 
    %Z_1 = \sum _{i=1}^{M} \sum _{t=1}^{M} y_{it} x_{it}, \\ 
    Z_{\text{OD}} = \arg \min_{\boldsymbol{c}_{q} \in C}} \sum_{i=1}^{M}\sum_{j=1}^{M} \hat{y}_{ij} s^{(\boldsymbol{c}_{q})}_{ij}, \quad \mbox{for} \ 1 \leq q \leq 2^n %q = 1, 2,\dots 2^n,
   \label{eq:assignment-problem-solution-permutation-ml}
\end{equation}
where $s^{(\boldsymbol{c}_{q})}_{ij}$ is each element in the permutation matrix produced by a codeword $\boldsymbol{c}$.

\section{Proposed Soft-Decision Decoder and Schemes}

\subsection{Branch and Bound}
In order to solve $\boldsymbol{Y}$ using branch and bound (BB) \cite{little-murty-sweeney-karel}, $\boldsymbol{Y}$ is divided into $M+1$ levels $\epsilon_i = \epsilon_0, \epsilon_1, \dots, \epsilon_M$ and each column is a node defined as $\delta_t = \delta_1, \delta_2, \dots, \delta_M$. Then, BB \cite{little-murty-sweeney-karel} is used as a SD technique to solve an assignment problem using a state space tree shown in Fig. \ref{fig:branch-and-bound-tree-diagram} with $M = 4$. At level 0, there exists an initial node containing all integers $\{c_1,c_2,\dots, c_M\}$ in no specific order and none of the $M$ jobs is yet assigned. For simplicity, the initial node for $M = 4$ is $1234$ and nodes $1/234$, $2/134$ up to $4/123$ are obtained at $\epsilon_1$. One node $\hat{\delta_{\epsilon_1}}$ at $\epsilon_1$ from the $M$ branches is scheduled if
\begin{figure}
    \centering\includegraphics[width=15pc]{diagrams/branch_and_bound_tree_space.eps}
    \caption{Tree-based method to decode permutation codes using branch and bound with $M = 4$.}
    \label{fig:branch-and-bound-tree-diagram}
\end{figure}
\begin{equation} 
    \hat{\delta}_{\epsilon_1} = \sum_{i=1}^{M} \min_{1 \leq j \leq M} (\hat{y}_{ij}). %\:\:\: 1 \leq t \leq M. %t = 1, 2,\dots,M.
    \label{branch-and-bound-level-0}
\end{equation}
The other nodes are pruned while the surviving node at $\epsilon_1$ satisfying (\ref{branch-and-bound-level-0}) is divided into $M-\epsilon_1$ branches at $\epsilon_2$. The node to be kept at this level satisfies
\begin{equation} 
    \hat{\delta}_{\epsilon_2} = \hat{y}_{1\hat{\delta}_{\epsilon_2}} + \sum_{i=2}^{M} \min_{\substack{1 \leq j \leq M, \\ \hat{y}_{i\hat{\delta}_{\epsilon_2}} = \infty} } (\hat{y}_{ij}). %:  %\: 2 \leq t \leq M, \;
    %\hat{y}_{i\hat{\delta}_{\epsilon_2}} = \infty. %t = 2,\dots,M, \; \hat{y}_{i\hat{\delta}_{\epsilon_2}} = \infty.
    \label{branch-and-bound-level-1}
\end{equation}
This process of pruning and branching is done until the last level $M$ or the $M-\epsilon_i$ level at which only one assignment is possible.

%\subsection{The Permutation Soft-Decision Decoder}
%The first iteration in the PSDD uses the HA to solve for $Z_1$ with steps described in \cite{kuhn} and a permutation code application in \cite{kolade-versfeld-van-wyk}. Murty's algorithm \cite{murty} ranks $Z_2, Z_3, \dots, Z_{2^n}$ and is used in the PSDD if the HA outputs a $\boldsymbol{c} \notin C$. Using the solution matrix from $Z_1$, $n-1$ non-empty subsets of $\boldsymbol{Y}$ form nodes $N_1, N_2, \dots, N_{n-1}$, by partitioning $a_1$. Nodes in this case are defined as $N_1 = {\{\overline{(1, j_1)}}\},N_2 = {\{(1, j_1), (\overline{2,j_2)}}\},\dots, N_{n-1} = {\{(1, j_1), \dots, \overline{(n-1, j_{n-1})}}\}$. Row-column pairs with the bar ($\overline{\cdot,\cdot}$) indicate row-column elements to be replaced with $\infty$ while row-column elements without the bar are removed from $\boldsymbol{Y}$. The minimum cost is then solved for each node and the node with the least cost forms the next assignment $a_2$.
%Alternatively, a brute force approach
%\begin{equation} 
%  \begin{aligned}
%  \label{eq:assignment-problem-modified}
%    Z_b = \sum_{i=1}^{M}\sum_{t=1}^{M} y_{it} x_{it}, \quad \mbox{for} \ 1 \leq b \leq |C|,
%  \end{aligned}
%\end{equation}
%ranks the cost of each codeword in $C$ and the permutation codeword corresponding to the lowest cost $Z_1$ is the ML performance of the soft-decision decoder.

%The PSDD decoder is iterative and always outputs a permutation codeword. It however checks if the output codeword $\boldsymbol{c} \in C$. The decoder iterates until either $\boldsymbol{c} \in C$ or it reaches the specified number of iterations.

%The next two sections discuss two methods of decoding the output of the PSDD. We discuss decoding the binary sequence using the Viterbi decoder and decoding the integer sequence using the modified Viterbi decoder.

\subsection{Schemes}
%The proposed decoding schemes apply an iterative soft-decision decoder to the soft output of the channel in order to produce a permutation sequence.
As shown in Fig. \ref{fig:decoder-sd}, the PSDD uses BB or HA and Murty algorithms to decode $\boldsymbol{Y}$, hence the dashed lines. The dotted lines around the Murty block indicates the Murty algorithm is only used when $\boldsymbol{c} \notin \boldsymbol{C}$ at HA. Otherwise, the Murty step is skipped.

\subsubsection{Scheme 1}
$\boldsymbol{Y}$ is decoded using HA and Murty and the resulting permutation sequence is decoded using the non-binary Viterbi decoder. If HA produces a sequence $\boldsymbol{c} \notin C$, Murty iterates until $\boldsymbol{c} \in C$ or the specified maximum number of iterations is reached. Therefore, more iterations increase the probability of forwarding a permutation sequence with zero Hamming distance with at least one transition path in the trellis of the Viterbi decoder. For large code books, the PSDD decodes with low complexity and the Viterbi decoder searches the path in the trellis that is exactly equal to $\boldsymbol{c}$.
%As shown in Fig. \ref{fig:decoder-sd}, this scheme combines HA and Murty iteratively to output a permutation sequence. The dotted line shows the two decoders which are BB and the combination of HA and Murty. The dashed box indicates Murty's algorithm is optional and iterative. The HA and Murty combine to decode $\boldsymbol{Y}$ iteratively such that HA runs the first iteration while Murty runs the second to the $g$-th iteration. The BB algorithm only runs one iteration. Since the output of the PSDD is always a permutation code, the PTC decoder decodes the sequence $\boldsymbol{c}$ produced from the PSDD. If we iterate in the PSDD until $\boldsymbol{c} \in C$, then the PTC is presented with a sequence of zero Hamming distance with at least one transition path in the trellis. For large permutation code books, the PSDD decodes with low complexity and the Viterbi decoder of the PTC searches the path that is exactly equal to $\boldsymbol{c}$. %Since more iterations increase the probability of $\boldsymbol{c} \in C$, the PTC decoder is supplied with a permutation codeword with high probability of zero $d_{min}$ with one codeword in $C$. Hard-decision Viterbi decoding using Hamming distance $d_m$ between $\hat{c}$ and paths in the trellis is then used to decode the permutation sequence.

\begin{figure}
\centering\includegraphics[width=20pc]{diagrams/system_model_decoder_sd.eps}
\caption{Decoder system model of permutation code soft-decision and permutation trellis decoder.}
\label{fig:decoder-sd}
\end{figure}

\subsubsection{Scheme 2}
Here, the Viterbi decoder is used to decode the binary output from the permutation to binary code demapper. The PSDD produces a permutation code $\boldsymbol{c}$ that is demapped to its binary equivalent.
%from the binary to permutation mapping table. 
If the final iteration of the PSDD produces a codeword $\boldsymbol{c} \notin C$, minimum distance decoding between $\boldsymbol{c}$ and all codewords in $C$ is performed before demapping. This binary output is then decoded normally using the Viterbi decoder. 

\subsubsection{Schemes 3 \& 4}
In Scheme 3, the channel output $\boldsymbol{Y}$ is decoded with BB to solve for $Z_1$. The permutation sequence produced is then forwarded to the non-binary Viterbi decoder. In Scheme 4, the permutation sequence produced by BB is demapped to its binary equivalent and forwarded to the binary Viterbi decoder, similar to Scheme 2. BB uses a single iteration, hence only $Z_1$ is solved in Schemes 3 and 4. 

%While Schemes 3 and 4 are similar to 1 and 2 respectively, the HA element of the PSDD is replaced with the BB algorithm to solve for $Z_1$. %The BB algorithm proposed and extensively described in \cite{little-murty-sweeney-karel} uses a tree-based method to solve $Z_1$. The item in each row of $\boldsymbol{Y}$ which satisfies the lower bound condition determines the items from the next row that will be included in the sub-tree. 
%Scheme 3 follows a similar pattern to scheme 1 where the permutation sequence at the output of the BB algorithm is decoded with the Viterbi algorithm. Scheme 4 on the other hand is similar to scheme 2 where the output of the BB algorithm is demapped using a mapping table, thereby producing a binary input to the Viterbi decoder.

%\begin{figure}
%\centering\includegraphics[width=20pc]{diagrams/system_model_decoder_sd_demapped.eps}
%\caption{Decoder system model of permutation code soft-decision, demapper and binary Viterbi decoder.}
%\label{fig:decoder-sd-demapped}
%\end{figure}

In the case of the PLC channel, the soft-decision algorithms can be applied after the threshold detector which applies $0.6\sqrt{E_m}$ on the each received symbol energy as described in \cite{ferreira-vinck-swart-beer}. As an example, consider a transmitted codeword 3214. The received permutation matrix $\boldsymbol{Y}_{\text{I}}$ affected by impulse noise at time $t_4$ can be represented as
\begin{equation}
  \label{eq:received-y-job-worker}
  \boldsymbol{Y}_{\text{I}} =
  \scalemath{0.7}{
  \begin{blockarray}{*{4}{c} l}
    \begin{block}{*{4}{>{$\footnotesize}c<{$}} l}
      t_1 & t_2 & t_3 & t_4 \\
    \end{block}
    \begin{block}{[*{4}{c}]>{$\footnotesize}l<{$}}
      0 & 0 & \fbox{1} & 1 \\
      0 & \fbox{1} & 0 & 1 \\
      \fbox{1} & 0 & 0 & 1 \\
      0 & 0 & 0 & \fbox{1} \\
    \end{block}
  \end{blockarray} } \text{ or } 
  \begin{equation}
  \label{eq:received-y-job-worker}
  \boldsymbol{Y}_{\text{N}} =
  \scalemath{0.7}{
  \begin{blockarray}{*{4}{c} l}
    \begin{block}{*{4}{>{$\footnotesize}c<{$}} l}
      t_1 & t_2 & t_3 & t_4 & \\
    \end{block}
    \begin{block}{[*{4}{c}]>{$\footnotesize}l<{$}}
      1 & 1 & \fbox{1} & 1 & f_1 \\
      0 & \fbox{1} & 0 & 0 & f_2 \\
      \fbox{1} & 0 & 0 & 0 & f_3 \\
      0 & 0 & 0 & \fbox{1} & f_4 \\
    \end{block}
  \end{blockarray} },
\end{equation}
when affected by NBI at $f_1$.
$\boldsymbol{Y}_{\text{I}}$ and $\boldsymbol{Y}_{\text{N}}$ can be easily solved using the PSDD to produce the codeword 3214 as shown by the boxed values. The codeword can then be either demapped to its binary equivalent or decoded with the non-binary sequence $\boldsymbol{c}$ using the Viterbi algorithm.

\section{Simulation Results and Complexity Analysis}
We compare the simulated BER of the modified non-binary PTC decoder in \cite{ferreira-vinck-swart-beer} with BERs obtained from the proposed decoding schemes discussed in Section III. %The results from the schemes are compared also with the existing "modified" PTC decoding algorithm described in \cite{ferreira-vinck-swart-beer}. The  proposed decoding schemes combine the performance of up to four iterations $g$ of the soft-decision decoder with the PTC or the Viterbi decoder. %For simplicity of reference, we refer to the scheme described in section III as scheme A while the scheme in section IV is referred to as scheme B. 
DIMs of PTC were simulated with two different codes of $R_{\text{C}} = 1/2$ mapped onto $M = 3$ and $R_{\text{C}} = 2/3$ mapped onto $M = 4$ code book. The former is generated from $K = 3$, minimum free distance of 9 and octal generator polynomial (7 5). The latter is generated from $K = 4$. %($[2, 2]$) 
The minimum free distance is 6 and the octal generator polynomial is (1 3 0; 3 2 3). These codes are then mapped onto distance increasing permutation code books of $M = 3$ and $M = 4$ respectively. %using the mappings shown in Tables \ref{table:1_2_3_mapping_table} and \ref{table:2_3_4_mapping_table} respectively. 
We define SNR per symbol $E_s/N_0$ as the ratio of the signal energy $E_s$ to noise power spectral density $N_0$. Therefore, the SNR per bit $E_b/N_0$ of the system for bit energy $E_b$ is defined as
\begin{equation} 
  \begin{aligned}
  \label{eq:snr-per-bit}
    \dfrac{E_b}{N_0} = \dfrac{E_s}{N_0 \times R_{\text{P}} \times \text{log}_{2}{M}}.
  \end{aligned}
\end{equation}

Results in Fig. \ref{fig:half-rate-awgn} show tight BER performance between the modified PTC decoder and the soft-decision schemes. When $M$ is increased in Fig. \ref{fig:two-third-rate-awgn-iterations}, the BER coding gains obtainable from the Schemes 1 and 2 become more evident with up to 3dB at $g = 4$. Figs. \ref{fig:quarter-rate-awgn} and \ref{fig:quarter-rate-plc} show significant BER improvement in AWGN and PLC channels respectively with Schemes 3 and 4 performing close to the OD of Schemes 1 and 2.

\subsection{BER Performance and $\frac{2^n}{M!}$ ratio}
The soft-decision decoders presented provide the advantage of always outputting a permutation of integers by solving an assignment problem. The soft-decision decoder's probability of producing a codeword $\boldsymbol{c} \in C$ can be described by the ratio $\frac{2^n}{M!}$. Hence, the performance of the schemes approaches the OD performance as $2^n$ increases. For example, in Figs. \ref{fig:quarter-rate-awgn} and \ref{fig:quarter-rate-plc} which use a convolutional code of $R_{\text{C}} = 1/4$, $K = 6$, an octal generator polynomial (53 67 71 75) and $M = n$, the $2^{M}$ unique binary sequences are mapped onto a code book with $M = 4$. Since $\frac{2^n}{M!} = 0.667$, each scheme of the soft-decision decoders is more likely to choose a codeword $\boldsymbol{c} \in C$. Fig. \ref{fig:quarter-rate-plc} uses the threshold detector discussed in Section II-C. The OD of Schemes 1 and 2 are not optimal at lower SNRs because of the \{0, 1\} cost matrix produced by the threshold detector. Hence, multiple assignments can produce the same highest cost and the resulting codeword, which may not belong in $C$ is randomly chosen.  For lower values of $2^n$ such as in Figs. \ref{fig:half-rate-awgn} and \ref{fig:two-third-rate-awgn-iterations}, more iterations such as $g = 4$ are required to produce $\boldsymbol{c} \in C$ compared to $g = 1$. 
Schemes 2 and 4 further improve the performance of the soft-decision because the demapping process chooses one of the $2^n$ possible binary sequences using Hamming distance decoding. Hence, the binary sequence forwarded to the Viterbi decoder follows a path in Viterbi's trellis with zero Hamming distance with the branches of the decoded path in the trellis. 
%the demapping step presented in Schemes 2 and 4 improve the BER performance at $g = 4$ because the likely transmitted codeword is demapped to its binary equivalent. Therefore, higher iterations such as $g = 4$ increase the chance of demapping to the correct encoded sequence, hence improving the accuracy of the Viterbi decoder.

\begin{figure}
\centering\includegraphics[width=20pc]{diagrams/results/ptc_rate_1_2_3_awgn}
\caption{BER comparing the four PSDD decoding schemes with the PTC decoder for $R_{\text{C}}$ = 1/2 and $M$ = 3 in AWGN channel.}
\label{fig:half-rate-awgn}
\end{figure}

\begin{figure}
\centering\includegraphics[width=20pc]{diagrams/results/ptc_rate_2_3_4_awgn.eps}
\caption{BER comparing the four PSDD decoding schemes with the PTC decoder for $R_{\text{C}}$ = 2/3 and $M$ = 4 in AWGN channel.}
\label{fig:two-third-rate-awgn-iterations}
\end{figure}

\begin{figure}
\centering\includegraphics[width=20pc]{diagrams/results/ptc_rate_1_4_4_awgn.eps}
\caption{BER comparing the four PSDD decoding schemes with the PTC decoder for $R_{\text{C}}$ = 1/4 and $M$ = 4 in AWGN channel.}
\label{fig:quarter-rate-awgn}
\end{figure}

\begin{figure}
\centering\includegraphics[width=20pc]{diagrams/results/ptc_rate_1_4_4_plc_0_1_threshold.eps}
\caption{BER comparing the four PSDD decoding schemes with the PTC decoder for $R_{\text{C}}$ = 1/4 and $M$ = 4 in AWGN and IN channel with $A$ = 0.1.}
\label{fig:quarter-rate-plc}
\end{figure}

%\begin{figure}
%  \begin{subfigure}[b]{0.24\textwidth}
%    \includegraphics[width=\textwidth, height=5.55cm, keepaspectratio]{diagrams/results/ptc_rate_1_4_4_awgn.eps}
%    \caption{BER comparison of schemes and PTC decoder for $R_{\text{C}}$ = 1/4 and $M$ = 4 in AWGN\\}
%    \label{fig:quarter-rate-awgn}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.24\textwidth}
%    \includegraphics[width=\textwidth]{diagrams/results/ptc_rate_1_4_4_plc_0_1_threshold.eps}
%    \caption{BER comparison of schemes and PTC decoder for $R_{\text{C}}$ = 1/4 and $M$ = 4 in AWGN and IN channel with $A$ = 0.1}
%    \label{fig:quarter-rate-plc}
%  \end{subfigure}
%\end{figure}

%\begin{figure}
%\centering\includegraphics[width=20pc]{diagrams/results/ptc_rate_1_4_4_rayleigh.eps}
%\caption{BER comparing the four PSDD decoding schemes with the PTC decoder for $R_{\text{C}}$ = 1/4 and $M$ = 4 in AWGN and Rayleigh fading channels.}
%\label{fig:quarter-rate-rayleigh}
%\end{figure}

\subsection{Complexity Analysis}
The HA and Murty's algorithm add a combined complexity of $O(M^3)$ and $O(M^3 \text{ln}^2(M))$ for BB for a fixed $M$. For a state sequence of length $T$, the HA and Murty's algorithm complexity becomes $O(TM^3)$ in Schemes 1 and 2. Similarly, a complexity of $O(TM^3 \text{ln}^2(M))$ is derived for Schemes 3 and 4. These complexities in the PSDD of Schemes 1-4 replace the $O(TM^2)$ complexity required by the ED. Table \ref{table:decoders_complexities_table} lists the complexity required by each decoding step in Fig. \ref{fig:decoder-sd}.
%The PTC decoder decodes the output of the envelope detector (ED), thereby combining complexities $O(n)$ and $O(\frac{T}{M}4^{K - k})$ respectively \cite{lin-costello}. $T$ is the number of states of the decoder and $n$ is the input size. 

\begin {table}[ht]
%\begin {table}
\begin{center}
    \caption {Time Complexity of Decoders}
\begin{tabular}{ >{\centering\arraybackslash}m{0.45in} >{\centering\arraybackslash}m{0.25in} >{\centering\arraybackslash}m{0.75in}>{\centering\arraybackslash}m{0.5in}>{\centering\arraybackslash}m{0.6in}}
  \toprule[1.25pt]

  \hline

  %\textbf{} & \textbf{ED} & \textbf{PSDD} & \textbf{Demapping} & \textbf{PTC} & \textbf{Viterbi} \\ 
  \textbf{} & \textbf{ED} & \textbf{PSDD} & \textbf{Demapping} & \textbf{Viterbi} \\ 

  \hline PTC Decoding & $O(TM^2)$ & 0 & 0 & $O(T\cdot4^{K - k})$\\
  \hline Scheme 1 & 0 & $O(TM^3)$ & 0 & $O(T\cdot4^{K - k})$\\
  \hline Scheme 2 & 0 & $O(TM^3)$ & $O(TM!)$ & $O(T\cdot4^{K - k})$\\
  \hline Scheme 3 & 0 & $O(TM^3 \text{ln}^2(M))$ & 0 & $O(T\cdot4^{K - k})$\\
  \hline Scheme 4 & 0 & $O(TM^3 \text{ln}^2(M))$ & $O(TM!)$ & $O(T\cdot4^{K - k})$\\
  \hline

%  \hline PTC Decoding & $O(TM)$ & 0 & 0 & $O(\frac{T}{M}4^{K - k})$ & 0 \\
%  \hline Scheme 1 & 0 & $O(TM^2)$ & 0 & $O(\frac{T}{M}4^{K - k})$ & 0\\
%  \hline Scheme 2 & 0 & $O(TM^2)$ & $O(T(M - 1)!)$ & 0 & $O(\frac{T}{n}4^{K - k})$\\
%  \hline Scheme 3 & 0 & $O(TM^2 \text{ln}^2(M))$ & 0 & $O(\frac{T}{M}4^{K - k})$ & 0\\
%  \hline Scheme 4 & 0 & $O(TM^2 \text{ln}^2(M))$ & $O(T(M - 1)!)$ & 0 & $O(\frac{T}{n}4^{K - k})$\\
%  \hline

    \bottomrule[1.25pt]
    \end{tabular}
\label{table:decoders_complexities_table}
\end{center}
\end {table}
The Viterbi decoder's complexity is given as $O(T\eta^2)$ for a state size of $\eta = 2^{K - k}$, hence a modified complexity of $O(T \cdot 4^{K - k})$ per $T$ block. Schemes 2 and 4 however require an additional complexity of $O(TM!)$ for demapping every $M$ input. In cases where the threshold detector is used, the SD decoder reduces the complexity of computing the trellis branch metric. This is because the classical decoder compares the demodulated matrix with all possible code matrices with a complexity of $O(M!)$ per codeword. This becomes impractical for large codebooks. However, the increase in the complexity of the PSDD and BB for larger codebooks is minimal in comparison.

\section{Conclusion}
The design of four decoding schemes which combine three optimization algorithms to improve the BER performance of the PTC decoder is presented. The complexities of the different components of the decoding schemes are also analyzed. Demapping the permutation sequence to its binary equivalent before decoding with the Viterbi decoder produces the best BER coding gain when compared to the PTC decoder. The BER coding gains obtained from the schemes increase as the ratio of the permutation code book length to all possible permutations increases. While the improved BER coding gain is at the expense of additional complexity, a reasonable trade-off can be considered when the permutation code book contains large codewords. While multi-tone $M$-FSK has been established to improve the data rate of the $M$-FSK scheme, future work will require techniques for increasing the data rate of permutation-coded $M$-FSK.

%$M$-FSK with permutation codes is recommended to mitigate the effect of narrowband noise such as in PLC channels. While it is expected that soft-decision schemes improves BER performance in general, the performance and analysis of PTC for low data rate applications will assist to improve the performance in such channel. 

\begin{thebibliography}{10}

\bibitem{chang-chen-klove-tsai}
Jen-Chun Chang, Rong-Jaye Chen, T.~Klove, and Shi-Chun Tsai.
\newblock Distance-preserving mappings from binary vectors to permutations.
\newblock {\em IEEE Transactions on Information Theory}, 49(4):1054--1059,
  April 2003.

\bibitem{ferreira-vinck}
H.~C. {Ferreira} and A.~J.~H. Vinck.
\newblock Interference cancellation with permutation trellis codes.
\newblock In {\em Vehicular Technology Conference Fall 2000. IEEE VTS Fall
  VTC2000. 52nd Vehicular Technology Conference (Cat. No.00CH37152)}, volume~5,
  pages 2401--2407 vol.5, Sep. 2000.

\bibitem{ferreira-vinck-swart-beer}
H.~C. Ferreira, A.~J.~H. Vinck, T.~G. Swart, and I.~de~Beer.
\newblock Permutation trellis codes.
\newblock {\em IEEE Transactions on Communications}, 53(11):1782--1789, Nov.
  2005.

\bibitem{kolade-versfeld-van-wyk}
O.~Kolade, J.~Versfeld, and M.~van Wyk.
\newblock {Soft-Decision} decoding of permutation block codes in {AWGN} and
  {Rayleigh} fading channels.
\newblock {\em IEEE Communications Letters}, 21(12):2590--2593, Dec 2017.

\bibitem{kuhn}
H.~W. Kuhn.
\newblock The {Hungarian} method for the assignment problem.
\newblock {\em Naval Research Logistics Quarterly}, 2(1-2):83--97, 1955.

\bibitem{little-murty-sweeney-karel}
J.~D.~C. Little, K.~G. Murty, D.~W. Sweeney, and C.~Karel.
\newblock An algorithm for the traveling salesman problem.
\newblock {\em Operations Research}, 11(6):972--989, March 1963.

\bibitem{murty}
K.G. Murty.
\newblock Letter to the editor — an algorithm for ranking all the assignments
  in order of increasing cost.
\newblock {\em Operations Research}, 16(3):682--687, 1968.

\bibitem{proakis}
J.~G. Proakis and M.~Salehi.
\newblock {\em Digital Communications}, pages 203--219, 846--849.
\newblock McGraw-Hill, fifth edition, 2008.

\bibitem{schaub}
T.~{Schaub}.
\newblock Spread frequency shift keying.
\newblock {\em IEEE Transactions on Communications}, 42(234):1056--1064,
  February 1994.

\bibitem{vinck}
A.~J.~H. Vinck.
\newblock Coding for a terrible channel.
\newblock In {\em EU-COST289 2nd Workshop Special Topics on 4G Technologies},
  pages 101--106, University of Duisburg-Essen, Germany, Jul. 8-9, 2005.

\bibitem{viterbi}
A.~{Viterbi}.
\newblock Error bounds for convolutional codes and an asymptotically optimum
  decoding algorithm.
\newblock {\em IEEE Transactions on Information Theory}, 13(2):260--269, April
  1967.

\end{thebibliography}
